One-step Diffusion with Distribution Matching Distillation

Diffusion models generate high-quality images but require dozens of forward passes. We introduce Distribution Matching Distillation (DMD), a procedure to transform a diffusion model into a one-step image generator with minimal impact on image quality. We enforce the one-step image generator match the diffusion model at distribution level, by minimizing an approximate KL divergence whose gradient can be expressed as the difference between 2 score functions, one of the target distribution and the other of the synthetic distribution being produced by our one-step generator. The score functions are parameterized as two diffusion models trained separately on each distribution. Combined with a simple regression loss matching the large-scale structure of the multi-step diffusion outputs, our method outperforms all published few-step diffusion approaches, reaching 2.62 FID on ImageNet 64x64 and 11.49 FID on zero-shot COCO-30k, comparable to Stable Diffusion but orders of magnitude faster. Utilizing FP16 inference, our model generates images at 20 FPS on modern hardware.

==> 03_background.tex <==
\MG{following a discussion with Richard, I am not sure we need any of this section.}
diffusion models are generative models trained to reverse a gaussian diffusion process~\cite{sohl2015deep,ho2020denoising, song2020score} that progressively diffuses a sample from a data distribution $x_0 \sim p_\text{data}(x)$ into white noise $x_t\sim\mathcal{n}(0, \mathbf{i})$ over $t>0$ time steps.
the marginal distribution at timestep $t\in[1, t]$ is
\begin{equation}
    \label{eq:forward_diffuse}
    q_t(x_t|x_0)\sim\mathcal{n}(\alpha_t x_0; \sigma_t^2,
\mathbf{i})
\end{equation}
where $\alpha_t$ and $\sigma_t$ are specified by a fixed noise schedule~\cite{karras2022elucidating, ho2020denoising}.
a trained diffusion model reverses this corruption process, i.e., it iteratively denoises samples $x_t$ from the tractable latent gaussian distribution into the desired data distribution.

\ty{for sd model, it is epsilon prediction, and i do the conversion using equation 4. moreover, the connection between score and diffusion is firstly based on epsilon prediction. so for completeness, let's keep both}
Common formulations of diffusion models include the noise prediction~$\epsilon_\theta(x_t, t)$ and the data prediction~$\mu_\theta(x_t, t)$ schemes~\cite{ho2020denoising, karras2022elucidating}.
These models operate as time-conditioned networks that progressively denoise an input corrupted by noise, where the level of noise variance is determined by the timestep $t$.
\MG{need to introduce the notation for the time-conditioned networks}
\TY{fixed}
Given a noisy image $x_t$, obtained by diffusing the real image $x$ with Gaussian noise $\epsilon$ and timestep $t$, the noise prediction model minimizes 

\begin{equation}
    \mathcal{L}_{noise} = w_t ||\epsilon_\theta(x_t, t) - \epsilon||^2
\end{equation}

\noindent 
while the data prediction model minimizes 

\begin{equation}    
\label{eq:diffusion_data}
    \mathcal{L}_{data} = w_t ||\mu_\theta(x_t, t) - x||^2 
\end{equation}

\noindent 
and $w_t$ is a timestep-dependent weighting. 
The noise prediction model and data prediction model could be converted to each other according to the following rule~\cite{karras2022elucidating} 

\begin{equation}
\small 
    \begin{aligned}
    \mu_\theta(x_t, t) &= \frac{x_t - \sigma_t \epsilon_\theta(x_t, t)}{\alpha_t } \quad
    \epsilon_\theta(x_t, t) = \frac{x_t - \alpha_t \mu_\theta(x_t, t)}{\sigma_t}
    \end{aligned}
\end{equation}

Moreover, Score-SDE~\cite{song2020score} shows that the diffusion model approximates the score function of the diffused distribution 

\begin{equation}
\label{eq:diffusion_score}
    \frac{x_t - \alpha_t \mu_\theta(x_t, t)}{\sigma_t} = \epsilon_\theta(x_t, t) \approx -\sigma_t \nabla_{x_t} \text{log} q_t(x_t)
\end{equation}

\paragraph{Classifier-Free Guidance.}
For text-to-image diffusion models, Classifier-Free Guidance~\cite{ho2022classifier} is widely used to improve the image quality. 
Given a guidance scale $\omega$, classifier-free guidance replaces the original noise prediction $\epsilon_\theta(x_t, t, c)$ with 
\begin{equation}
\label{eq:cfg}
    \epsilon'_\theta(x_t, t) = \epsilon_\theta(x_t, t, \varnothing) + \omega \times(\epsilon_\theta(x_t, t, c) - \epsilon_\theta(x_t, t, \varnothing))
\end{equation}
\noindent 
where $c$ and $\varnothing$ represents the text and null embedding respectively.   


